Meteor statistics I: The distribution of instrumental magnitudes

The distribution of meteor magnitudes is known to follow an exponential distribution, where the base of this distribution is called the population index. The distribution of observed magnitudes preserves this behavior, but is truncated by the detection threshold. If both the population index and detection threshold can be determined, observed meteor rates can be converted to fluxes and extrapolated to any desired brightness or size. We argue that the distribution of observed or instrumental meteor magnitudes is best modeled as an exponentially modified Gaussian (exGaussian) distribution. This is for three reasons: first, an exGaussian distribution is the natural result of random variations in detection threshold and/or post-detection measurement errors in magnitude. Second, an exGaussian distribution provides a better fit to the magnitude distribution than all other competing distributions in the literature; we demonstrate this using both a set of faint optical meteor magnitudes and a set of radar meteor echo amplitudes. Finally, the population index, mean detection threshold, and random variation/error terms are easily extracted from the best-fit parameters of an exGaussian distribution.

==> abstract.tex <==
The distribution of meteor magnitudes is known to follow an exponential distribution, where the base of this distribution is called the population index. The distribution of observed magnitudes preserves this behavior, but is truncated by the detection threshold. If both the population index and detection threshold can be determined, observed meteor rates can be converted to fluxes and extrapolated to any desired brightness or size. We argue that the distribution of observed or instrumental meteor magnitudes is best modeled as an exponentially modified Gaussian (exGaussian) distribution. This is for three reasons: first, an exGaussian distribution is the natural result of random variations in detection threshold and/or post-detection measurement errors in magnitude. Second, an exGaussian distribution provides a better fit to the magnitude distribution than all other competing distributions in the literature; we demonstrate this using both a set of faint optical meteor magnitudes and a set of radar meteor echo amplitudes. Finally, the population index, mean detection threshold, and random variation/error terms are easily extracted from the best-fit parameters of an exGaussian distribution.

